Seeing What You Say: Expressive Image Generation from Speech

This paper proposes VoxStudio, the first unified and end-to-end speech-to-image model that generates expressive images directly from spoken descriptions by jointly aligning linguistic and paralinguistic information. At its core is a speech information bottleneck (SIB) module, which compresses raw speech into compact semantic tokens, preserving prosody and emotional nuance. By operating directly on these tokens, VoxStudio eliminates the need for an additional speech-to-text system, which often ignores the hidden details beyond text, e.g., tone or emotion. We also release VoxEmoset, a large-scale paired emotional speech-image dataset built via an advanced TTS engine to affordably generate richly expressive utterances. Comprehensive experiments on the SpokenCOCO, Flickr8kAudio, and VoxEmoset benchmarks demonstrate the feasibility of our method and highlight key challenges, including emotional consistency and linguistic ambiguity, paving the way for future research.

==> fig_tex/teaser.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/aaai_teaser.pdf}
    \vspace{-2em}
    \caption{\small{Generated samples by \ours on \oursbench. Each image embodies the nuanced effect conveyed in the spoken prompt.}}
    \label{fig:teaser}
\end{figure}

==> table/class.tex <==
\begin{table}[t]
    \caption{Number of images per emotion category in \oursbench.}\label{app:class}
    
    \centering
    \small
    \begin{tabular}{lc}
        \toprule
        Category & \# Images \\
        \midrule
        Enjoyment & 37,302 \\ 
        Anger & 10,141 \\ 
        Disgust & 10,128 \\ 
        Fear & 12,760 \\ 
        Sadness & 12,063 \\
        \midrule
        Total & 82,394 \\ 
        \bottomrule
    \end{tabular}
        
\end{table}
% {'enjoyment': 111906, 'anger': 30423, 'disgust': 30384, 'fear': 38280, 'sadness': 36189}

==> table/prompt.tex <==
\begin{table}[t]
    % \vspace{-1em}
    \caption{Text prompt used to make captions with LLaVA-OV.}\label{tab:prompt}
    
    \centering
    \small
    % \resizebox{\linewidth}{!}{
    \begin{tabularx}{\linewidth}{X}
        \toprule
        \textit{Generate three disjoint captions for the given image. Each caption should:} \\
        \textit{* Have a different sentence structure,} \\ 
        \textit{* Avoid emotional expressions or subjective interpretations,} \\
        \textit{* Describe different aspects of the image, such as objects, actions, spatial relationships, or surroundings,} \\
        \textit{* Be between 8 and 15 words long,} \\
        \bottomrule
    \end{tabularx}
    % }
\end{table}

